Network Sampling Methods for Estimating Social Networks, Population Percentages, and Totals of People Experiencing Unsheltered Homelessness

In this article, we propose using network-based sampling strategies to estimate the number of unsheltered people experiencing homelessness within a given administrative service unit, known as a Continuum of Care. We demonstrate the effectiveness of network sampling methods to solve this problem. Here, we focus on Respondent Driven Sampling (RDS), which has been shown to provide unbiased or low-biased estimates of totals and proportions for hard-to-reach populations in contexts where a sampling frame (e.g., housing addresses) is not available. To make the RDS estimator work for estimating the total number of people living unsheltered, we introduce a new method that leverages administrative data from the HUD-mandated Homeless Management Information System (HMIS). The HMIS provides high-quality counts and demographics for people experiencing homelessness who sleep in emergency shelters. We then demonstrate this method using network data collected in Nashville, TN, combined with simulation methods to illustrate the efficacy of this approach and introduce a method for performing a power analysis to find the optimal sample size in this setting. We conclude with the RDS unsheltered PIT count conducted by King County Regional Homelessness Authority in 2022 (data publicly available on the HUD website) and perform a comparative analysis between the 2022 RDS estimate of unsheltered people experiencing homelessness and an ARIMA forecast of the visual unsheltered PIT count. Finally, we discuss how this method works for estimating the unsheltered population of people experiencing homelessness and future areas of research.

==> cuttingBoard.tex <==
%%%%%%%%%%%%%
%% Helpful
%%%%%%%%%%%%

It is assumed that the author is familiar with either plain
\TeX, \AmS-\TeX{} or a standard \LaTeX\ setup and, hence,
only the essential points are described in this document.
Nevertheless, we hope that this document is generally sufficient
for describing the requirements for preparation of
manuscripts. For more details, please see the \textit{\LaTeX{} User's Guide} or
\textit{The not so short introduction to \LaTeXe}.


\section{Installation}
\label{sec2}

Provided with \verb+ouparticle.cls+ are the files
\verb+sample.tex+ (this document explains the various
features of \verb+ouparticle.cls+) and \verb+sample.pdf+
(how the output using \verb+sample.tex+ should be). Your
paper can be compiled with standard \LaTeX,
preferably with the current \LaTeXe\ version. It will probably work
with older versions of \LaTeXe; however, this has not been
tested. The file \verb+ouparticle.cls+ needs to be copied
into a directory where \TeX\ looks for input files. The other files
need to be kept as a reference while preparing
your manuscript. Please use the predefined commands from \verb+sample.tex+ for title,
authors, abstract, body, etc.


\section{Preparing your manuscript}
\label{sec3}

\subsection{General guidelines}
\label{sec3.1}

\begin{enumerate}
\item
\LaTeX\ and \AmS-\LaTeX\ provide a rich set of commands for all common, important
features of your paper. Use them; avoid definitions and use of custom commands.

\item
There is no need to redefine any \TeX, \LaTeX\ or \AmS-\LaTeX\ commands.

\item
Avoid direct formatting for headings cleanly set as section headings.

\item
Use \LaTeX\ commands for font changes. For example: use \verb+\textbf{phrase}+,
not \verb+{\bf phrase}+; use \verb+\mathcal{C}+, not \verb+{\cal C}+; etc.
\end{enumerate}


\subsection{How to start with \texttt{ouparticle.cls}}
\label{sec3.2}

Before you type anything that actually appears in the paper, you need to
include a \verb+\documentclass{ouparticle}+ command at the very beginning,
and then the two commands that have to be part of any \LaTeX\ document,
\verb+\begin{document}+ at the start and \verb+\end{document}+ at the
end of your paper.


\subsection{Document structure}
\label{sec3.3}

The main structure of your paper is as follows:

\begin{verbatim}
\documentclass[12pt,...]{ouparticle}
\usepackage[...]{packages}

\title{...}
\author{
    \name{...}
    \address{...}
    \email{...}
        \and
    \name{...}
    \address{...}
    \email{...}
        \and
    \name{...}
    \address{...}
    \email{...}
}
\abstract{...}
\keywords{...}

\maketitle

\begin{document}

\section{....}
...
\subsection{....}
....
\end{document}
\end{verbatim}


\subsection{Options}
\label{sec3.4}

By default, all of the options within \verb+article.cls+ are available
with this class file. This class file provides the following additional options.

\begin{description}
\item \textbf{oneline:}
This option will set your entire manuscript in one line spacing.
It will not affect the footnote, figure and table environments.

\item \textbf{halfline:}
This is to set your entire manuscript in half line spacing.

\item \textbf{endnotes:}
To make all footnotes to endnotes. You may follow the same
coding \verb+\footnote{text}+ for both footnotes and endnotes. Once you use this option
you have to use the \verb+\theendnotes+ command at the place where all the endnotes
have to be set in your paper.

\item \textbf{numbib:}
This is the default option that numbers the bibliography items;
this option does nothing with natbib and other packages.

\item \textbf{nonumbib:} For unnumbered bibliography.
\end{description}


\subsection{Front matter}
\label{sec3.5}

The title of the manuscript is simply specified by using the \verb+\title{text}+ command in
the same manner as in this sample. Author's information consists of the name of the author
and the corresponding institutions with addresses, as given in this example. Include an
electronic mail address if available, inserting it into the \verb+\email{text}+ commands.
You may follow the same coding if there are more than one author; separate authors with
\verb+\and+. Please identify the corresponding author with his/her electronic
mail address by \verb+\thanks{text}+. An abstract for your paper is specified by using
\verb+\abstract{text}+. A \verb+\keywords{text}+ macro may also be used to indicate keywords for the
article. Use \verb+\maketitle+ after the abstract and keywords to make the header of your article.

\subsection{Sections and subsections}
\label{sec3.6}

To begin a new section, give the heading of that section in the \verb+\section{text}+ command.
A section number is supplied automatically. Use the starred form (\verb+\section*{text}+) of the
command to suppress the automatic numbering. If you want to be able to make reference to that section,
then you need to \texttt{label} it (see Section \ref{sec3.14}). You can have sections up to
five levels. The sectioning commands are \verb|\section|, \verb|\subsection|, \verb|\subsubsection|,
\verb|\paragraph| and \verb|\subparagraph|.

\subsection{Ordinary text}
\label{sec3.7}

The ends of words and sentences are marked by spaces. It does not matter how many
spaces you type. The end of a line counts as a space. One
or more blank lines denote the end of a paragraph.

There are a number of things for which you need to follow different
methods. As you know, quotation marks, quotes within quotes,
dashes, ellipsis, etc. should be as per the \LaTeX\ standard input. \LaTeX\ interprets some
common characters as commands, and therefore you must instead type those common characters as
specific \LaTeX\ commands to generate them. Those characters are \$, \&, \%, \#, \{, and \}.

\subsection{Formatting}
\label{sec3.8}

One should always use \LaTeX\ macros rather than the lower-level
\TeX\ macros like \verb+\it+, \verb+\bf+ and \verb+\tt+. The
\LaTeX\ macros offer much improved features. The following table summarizes the font
selection commands in \LaTeX.


\subsubsection*{\LaTeX\ text formatting commands}
\begin{tabular}{ll@{\hskip60pt}ll}
\verb+\textit+  & Italics      &\verb+\textsf+  & Sans Serif\\
\verb+\textbf+  & Boldface     &\verb+\textsc+  & Small Caps\\
\verb+\texttt+  & Typewriter   &\verb+\textmd+  & Medium Series\\
\verb+\textrm+  & Roman        &\verb+\textnormal+ & Normal Series\\
\verb+\textsl+  & Slanted      &\verb+\textup+  & Upright Series
\end{tabular}


\subsubsection*{\LaTeX\ math formatting commands}
\begin{tabular}{ll@{\qquad}ll}
\verb+\mathit+     & Math Italics            &\verb+\mathfrak+   & Fraktur\\
\verb+\mathbf+     & Math Boldface       &\verb+\mathbb+     & Blackboard Bold\\
\verb+\mathtt+     & Math Typewriter     &\verb+\mathnormal+ & Math Normal\\
\verb+\mathsf+     & Math Sans Serif     &\verb+\boldsymbol+ & Bold math for Greek letters\\
\verb+\mathcal+    & Calligraphic        &                   & and other symbols
\end{tabular}


\subsection{Figures and tables}
\label{sec3.9}

Use normal \LaTeX\ coding for figures and tables.
Figure and table environments should be inserted after (not in) the paragraph in which
the figure is first mentioned or grouped all
together at the end of the file. They will be numbered automatically.
The following is an example of typesetting a table.

\begin{verbatim}
\begin{table}
\caption{Table caption text.}
\label{key}
The table matter goes here.
\end{table}
\end{verbatim}

As always with \LaTeX, the \verb+\label+ must be after the
\verb+\caption+, and inside the figure or table environment. The reference for
figures and tables inside text can be made using the \verb|\ref{key}| command.


\subsection{Equations}\label{sec3.10}

Equations are used in the same way as described in the \LaTeX\ manual.
Do not start a paragraph with a displayed equation. Equations are numbered consecutively, with equation numbers
in parentheses flush right.
 For example, if you type
\begin{verbatim}
\begin{equation}\label{eq1}
\int^{r_2}_0 F(r,\varphi){\rm d}r\,{\rm d}\varphi = [\sigma r_2/(2\mu_0)]
\int^{\infty}_0\exp(-\lambda|z_j-z_i|)\lambda^{-1}J_1 (\lambda r_2)J_0
(\lambda r_i\,\lambda {\rm d}\lambda)
\end{equation}
\end{verbatim}
then you will get the following output:
\begin{equation}\label{eq1}
\int^{r_2}_0 F(r,\varphi){\rm d}r\,{\rm d}\varphi = [\sigma r_2/(2\mu_0)]\int^{\infty}_0
\exp(-\lambda|z_j-z_i|)\lambda^{-1}J_1 (\lambda r_2)J_0 (\lambda r_i\,\lambda {\rm d}\lambda)
\end{equation}
It inserts space both above and below the equation. \AmS-\LaTeX{} has several environments that
make it easier to typeset complicated multiline displayed equations. These are explained in the
\AmS-\LaTeX{} User Guide. A \verb+subequation+ environment is available to create equations with
sub-numbering of the equation counter. It takes one (optional)
argument to specify the way that the sub-counter should appear.


\subsection{Displayed text}
\label{sec3.11}

Text is displayed by indenting it from the left and right margins.
Quotations are commonly displayed. There are short
quotations:
\begin{quote}
   This is a short quotation.  It consists of a
   single paragraph of text.  See how it is formatted.
\end{quote}
and longer ones:
\begin{quotation}
   This is a longer quotation.  It consists of two
   paragraphs of text, neither of which are
   particularly interesting.

   This is the second paragraph of the quotation.  It
   is just as dull as the first paragraph.
\end{quotation}
You can even display poetry.
\begin{verse}
   There is an environment
    for verse \\             % The \\ command separates lines
   Whose features some poets % within a stanza.
   will curse.

                             % One or more blank lines separate stanzas.

   For instead of making\\
   Them do \emph{all} line breaking, \\
   It allows them to put too many words on a line when they'd rather be
   forced to be terse.
\end{verse}


\subsection{Listings}
\label{sec3.12}

Another frequently displayed structure is a list. The
following is an example of an \emph{itemized} list.
\begin{itemize}
   \item This is the first item of an itemized list.
         Each item in the list is marked with a
         `$\bullet$'.

   \item This is the second item of the list. It
         contains another list nested inside it. The
         inner list is an \emph{enumerated} list.
         \begin{enumerate}
            \item This is the first item of an enumerated
                  list that is nested within the
                  itemized list.

            \item This is the second item of the inner list.
                  \LaTeX\ allows you to nest lists
                  deeper than you really should.
         \end{enumerate}
         This is the rest of the second item of the
         outer list. It is no more interesting than
         any other part of the item.
   \item This is the third item of the list.
\end{itemize}


\subsection{Displayed sentences: theorems and such}
\label{sec3.13}

These environments have to be defined with the help of \LaTeX's \verb+\newtheorem+ command, and
also with the \AmS-\LaTeX\ package for theorems that is already with your class file.
For example, \verb+\newtheorem{thm}{Theorem}+. Predefined theorem styles can be used in your article
to differentiate the theorem-like environments. You can have an extra command, \verb+\newproof+,
that can be used for displayed text. The following is an example of using the above-defined
\verb+thm+ environment.
\begin{verbatim}
\begin{thm}
This is body matter for this environment.
\end{thm}
\end{verbatim}

\subsection{Cross-referencing}
\label{sec3.14}

\LaTeX\ possesses features for labelling and cross-referencing
section headings, equations, tables, figures and theorems.
Their proper usage in the context of section headings, equations,
tables and figures are discussed in the appropriate sections.

Cross-referencing depends upon the use of `keys' that are defined by the user.
The \verb+\label{key}+ command is used to identify the links. Keys are strings of
characters that serve to label section headings, equations, tables and figures
that replace explicit, by-hand numbering. The \verb+\ref{key}+ command is used for
cross-referencing.

Files that use cross-referencing (and almost all manuscripts do)
need to be processed through \LaTeX\ at least twice to
ensure that the keys have been properly linked to the appropriate numbers.

\subsection{Footnotes and endnotes}
\label{sec3.15}

The footnote text can either appear at the bottom of a page or at the end of your paper.
The \verb+\footnote+ macro \emph{should not} be used in the front matter to provide additional
information about authors (such as corresponding addresses); instead, use \verb+\thanks{text}+ commands.
The document option `\texttt{endnotes}' is used to make endnotes. The command \verb+\theendnotes+ should
be used to place the endnotes at the required location in the text. They will be put in a separate
`Notes' section.


\subsection{Appendix}
\label{sec3.16}

The \verb+\appendix+ command signals that all following sections are
appendices, and therefore the headings after \verb+\appendix+ will be set
as appendix headings. For a single appendix, use \verb+\appendix*+ followed by the \verb+\section{text}+
command to suppress the appendix letter in the section heading.


\subsection{Special sections for notes and acknowledgements}
\label{sec3.17}

If you wish to include a `Notes' or `Acknowledgements' section in your paper,
use the \verb+\begin{notes}...\end{notes}+ macro. We use the same environment for both
`Notes' and `Acknowledgements'. The following examples show to how to use this macro.
\begin{verbatim}
\begin{notes}
Please note that this class file is provided as it is, and
copyright by Oxford University Press. You are free to use this
class file, provided that you do not make changes in this class file.
If you do make changes, you are requested to rename the class file.
\end{notes}

\begin{notes}[Acknowledgements]
The authors would like to thank...
\end{notes}

\end{verbatim}


\subsection{References}
\label{sec3.18}

The reference entries can be \LaTeX\ typed bibliographies or generated through a BIB\TeX\ database.
BIB\TeX\ is an adjunct to \LaTeX\ that aids in the preparation of bibliographies. BIB\TeX\
allows authors to build up a database or collection of bibliography entries that may be used for many
manuscripts. They also save us the trouble of having to specify formatting. More details can be found
in the \textit{BIB\TeX\ Guide}. For \LaTeX\ reference entries use the
\verb+\begin{thebibliography}....\end{thebibliography}+ environment (see below) to make references in your paper.
We have provided the class file option to distinguish two styles of references. Those options are \verb+numbib+ and \verb+nonumbib+.
You can select one of these options with the \verb+\documentclass+ command. By default the class file will take the
\verb+numbib+ option. The following is an example of \LaTeX\ bibliography.

\begin{verbatim}
\begin{thebibliography}{0}
\bibitem{bib1}
Goossens, M., F. Mittelbach, and A. Samarin: {\em The {\LaTeX} Companion}.
Addison-Wesley, Reading, MA, USA, 1994.
\bibitem{bib2}
Knuth, D.E: {\em The {\TeX}book}. Addison-Wesley, Reading, MA, USA, 1984.
\bibitem{bib3}
Lamport, L.: {\em {\LaTeX} -- A Document Preparation System -- User's
Guide and Reference Manual}. Addison-Wesley, Reading, MA, USA, 1985.
\bibitem{bib4}
Smith, I.N., R.S. Johnes, and W.P. Hines: 1992, `Title of the Article',
\textit{Journal Title in Italics} \textbf{Vol. no. X}, pp. 00--00
\end{thebibliography}
\end{verbatim}


\section{Macro packages}
\label{sec4}

The following packages are compulsorily needed by the class file:
\begin{verbatim}
amsmath         graphicx
amssymb         endnotes
amsfonts        setspace
verbatim        geometry
\end{verbatim}

The commonly used packages already used by this class file that authors can use whenever required are:
\begin{verbatim}
xspace          latexsym        url
amscd           multicol        algorithm
rotating        array           subfigure
\end{verbatim}

Additionally, you can use other packages and these should be loaded
using the \verb+\usepackage+ command.



Conventional homeless surveys and enumerations may be missing a substantial portion of the homeless population, qualifying this ‘hidden’ subpopulation as one of the most hard-to-count. 

Counting the number of people experiencing homelessness is challenging due to methodological inconsistencies such as varied definitions and inclusion criteria (Institute of Medicine (US) Committee on Health Care for Homeless People 1987), as well as factors related to the inherent inaccessibility of homeless populations. 

These factors include the transient or mobile nature of homeless populations, unstable living situations, and social stigma which inhibits people from revealing their housing status due to potential association with illegal or socially-disfavored activities (Heckathorn 1997; Khan et al. 2018; Metraux et al. 2016). 

This is especially problematic as homelessness in the United States has significantly increased since the recession in the 1980’s, while shelters and services have become insufficient in number for addressing the need. 

Demographics of this population have also become more widely varied, including people from backgrounds, ages, genders, and parts of the country not previously recognized in significant numbers (Lee-Anderson 2019). 

Hard-to-count populations have been traditionally estimated using indirect methods, such as shelter-use statistics, leading to inherently imperfect results (Berry 2007). Thus, as the homeless crisis has worsened, there have been increasing calls for improving the accuracy of counting methods to most effectively project service needs and distribute resources (Institute of Medicine (US) Committee on Health Care for Homeless People 1987).

This point-in-time count approach is conducted in the way that staff and volunteers go to homeless shelters and unsheltered places (e.g., street, abandoned buildings) to count homeless persons under a list of specifics, typically on a single night during the last ten days of January. For details and exceptions, please refer to the PiT Count Methodology Guide (U.S. Department of Housing and Urban Development (2014)) by HUD. In practice, the PiT count consist of sheltered homeless counts (e.g., the number of homeless persons who stay at emergency shelters, transitional housing projects, and so on) and unsheltered homeless counts (e.g., the number of homeless persons that sleep on streets and any other places that are not meant for human habitation). In addition to conducting the homeless PiT counts, volunteers and staff are also trained to interview homeless persons in order to collect information that is more detailed on demographic characteristics. When a CoC covers a large geographic area, it becomes very costly or even unfeasible to interview every single homeless person encountered. In such a case, a sampling approach is allowed to select subjects to be interviewed. In a complete data set of homeless PiT counts provided by HUD each year, it consists of the total counts, followed by sheltered and unsheltered counts, and counts for various demographic characteristics such as gender, race, age group, veteran, chronic homeless, and so on. 
The PiT Count Methodology Guide provides instructions for different sampling strategies on minimizing biases in the results when interviewing homeless persons for demographic information. However, it does not cover details of sampling on a subpopulation of a certain characteristic (e.g., youth, veterans, females). The research by Golinelli et al. (2015) shows how sampling the homeless youth from few locations or site types (even sites with the highest homeless youth concentration) can result in biases in the demographic characteristics for the population estimates. When sampling is needed, it usually calls for a case-by-case strategy due to the nature of human behaviors. The point of their case study though is that it is a call out for new and better sampling methods like those proposed in this grant.
